Mapping our Universe in 3D with MITEoR

Mapping our universe in 3D by imaging the redshifted 21 cm line from neutral hydrogen has the potential to overtake the cosmic microwave background as our most powerful cosmological probe, because it can map a much larger volume of our Universe, shedding new light on the epoch of reionization, inflation, dark matter, dark energy, and neutrino masses. We report on MITEoR, a pathfinder low-frequency radio interferometer whose goal is to test technologies that greatly reduce the cost of such 3D mapping for a given sensitivity. MITEoR accomplishes this by using massive baseline redundancy both to enable automated precision calibration and to cut the correlator cost scaling from N^2 to NlogN, where N is the number of antennas. The success of MITEoR with its 64 dual-polarization elements bodes well for the more ambitious HERA project, which would incorporate many identical or similar technologies using an order of magnitude more antennas, each with dramatically larger collecting area.

==> qaz <==
\author{Jeff Haoxuan Zheng}
\author{Max Tegmark}
\author{Victor Buza}
\author{Josh Dillon}
\author{Hrant Gharibyan}
\author{Jack Hickish}
\author{Eben Kunz}
\author{Adrian Liu}
\author{Scott Morrison}
\author{Jon Losh}
\author{Andy Lutomirski}
\author{Sruthi Narayanan]
\author{Ashley Perko}
\author{Devon Rosner}
\author{Nevada Sanchez}
\author{Katelin Schutz}
\author{Shana Tribiano}
\author{Matias Zaldarriaga}
\author{Kris Zarb-Adami}
\author{Ioana Zelko}
\author{Kevin Zheng}
\author{Richard Armstrong}
\author{Richard Bradley}
\author{Matt Dexter}
\author{Aaron Ewall-Wice}
\author{Qinxuan Pan}
\author{Magro, Allessio}
\author{Michael Matejek}
\author{Edward Morgan}
\author{Abraham Neben}
\author{Courtney Peterson}
\author{Joel Villasenor}
\author{Hung-I Yang}
\author{Christopher Williams}










